Automatic Evaluation of Attribution by Large Language Models

A recent focus of large language model (LLM) development, as exemplified by generative search engines, is to incorporate external references to generate and support its claims. However, evaluating the attribution, i.e., verifying whether the generated statement is fully supported by the cited reference, remains an open problem. Although human evaluation is common practice, it is costly and time-consuming. In this paper, we investigate the automatic evaluation of attribution given by LLMs. We begin by defining different types of attribution errors, and then explore two approaches for automatic evaluation: prompting LLMs and fine-tuning smaller LMs. The fine-tuning data is repurposed from related tasks such as question answering, fact-checking, natural language inference, and summarization. We manually curate a set of test examples covering 12 domains from a generative search engine, New Bing. Our results on this curated test set and simulated examples from existing benchmarks highlight both promising signals and challenges. We hope our problem formulation, testbeds, and findings will help lay the foundation for future studies on this important problem.

==> 1_Introduction.tex <==

\section{Introduction}
Generative large language models (LLMs) \cite[inter alia]{brown2020language,ouyang2022training,wei2022finetuned,chowdhery2022palm,openai2023chatgpt,openai2023gpt4,touvron2023llama} often struggle with producing factually accurate statements, resulting in hallucinations \cite{maynez2020faithfulness,ji2023survey}. Such hallucination can be a serious problem, especially in high-stakes domains such as healthcare \cite{nature_medicine_2023,lee2023benefits,lee2023AI} and finance \cite{wu2023bloomberggpt}, where factual accuracy is essential. 
 
Recent work attempts to address this issue by augmenting LLMs \cite{mialon2023augmented} with external tools \cite{schick2023toolformer,li2023api,qin2023tool} such as retrievers \cite{shuster2021retrieval,izacard2021leveraging,borgeaud2022improving} and search engines \cite{nakano2021webgpt,thoppilan2022lamda,glaese2022improving,shuster2022blenderbot}.
By presenting a generated statement with cited references to the user, an LLM is implicitly making a claim that its generated statement is attributable to the reference. 
However, \textit{how accurate is this attribution?}
% By incorporating external references, LLMs are expected to produce more accurate and up-to-date generations that are hopefully attributable to the external source. 
Concurrent work \cite{liu2023evaluating} finds that
such attributed LLMs are far from perfect from an attribution perspective---only 51.5\% of generations from four generative search engines are fully supported by their cited references. 
Inaccurate attribution could deceive users and further undermine the trustworthiness of LLMs. 
Therefore, it is critical to continually evaluate the attribution by LLMs.\footnote{The word ``attribution'' in this paper primarily refers to  ``the act of attributing something''. ``Evaluating attribution'' is synonymous to ``evaluating verifiability''  in \cite{liu2023evaluating}. }  

However, evaluating attribution \cite{rashkin2021measuring,gao2022attributed,bohnet2022attributed} is a challenging task, and existing work typically relies on human verification, which can be costly and time-consuming. For example, the average cost of annotating a single query-response-attribution example is around \$1 as reported by \citet{liu2023evaluating}. 
% Traditional generation metrics, such as embedding matching \cite{zhang2020bertscore} and n-gram matching \cite{shuster2021retrieval}, evaluate the quality of the generated text in terms of fluency, coherence, and relevance, without explicitly considering the attribution aspect. 
Consequently, there is a pressing need for a reliable automatic evaluation metric to measure the attribution by LLMs.


\begin{figure*}[!t]
    \centering
    \includegraphics[width=\linewidth]{AttrScore.pdf}
    \caption{\score~automatically evaluates attribution by LLMs. We show two recipes for implementing \score: (1) prompting LLMs, and (2) fine-tuning smaller LMs on repurposed datasets from related tasks. }
    %\hs{would it be better to put (1) and (2) before the two ways in the figure?}}
    \label{fig:attributionscore}
\end{figure*}


% 1. The main contribution is not very clear in the writing. For this specific work, you need to make a contribution list at the end of intro and keep echoing back and strengthening it throughout the paper. I suppose it's 1) formal definition of the problem and differentiation with related problems, 2) modeling development, including repurposing of existing datasets, 3) test sets (really need a name), evaluation, and insights

In this paper, we study the  \textit{automatic evaluation of attribution} and present a metric called \score \hsun{this is one part I am most uncertain about: Do we really want to call it `metric' or `score', given the current design? see comments in Table 2 as well.}, which measures how attributable a model's generation is to its reference (see Figure \ref{fig:attributionscore}). We first extend the definition of attribution to include two types of attribution errors: contradictory errors and extrapolatory errors, where the former means the generation directly contradicts the reference, and the latter means that there lacks sufficient information in the reference to determine the correctness of the generation. 
We explore two approaches for implementing \score: prompting LLMs and fine-tuning smaller LMs. For the fine-tuning approach, we repurpose data from similar tasks such as question answering (QA), fact-checking, natural language inference (NLI), and summarization. To facilitate the evaluation of attribution, we manually curate a set of test examples covering 12 different domains from the generative search engine New Bing.\footnote{\url{https://www.bing.com/new}}

% introduce two test sets: \textit{AttrEval-Simulation} and \textit{AttrEval-GenSearch}. The former includes simulated error examples created by modifying the context or the answer in existing benchmark QA datasets, while the latter includes a small set of annotated samples covering . 

Our quantitative results show that both prompting LLMs and fine-tuning smaller LMs achieve reasonable performance on curated and simulated test sets. However, our qualitative analysis reveals that automatic evaluation of attribution remains challenging, and most evaluation failures stem from three factors: insensitivity to fine-grained information comparisons such as overlooking contextual cues in the reference, insensitivity to fine-grained information comparisons such as numerical values, and failures in performing symbolic operations such as verifying set relationships. Based on these observations, we suggest two potential directions for improving \score: training \score to be more strongly conditioned on the reference, and augmenting the evaluation with external tools for different types of numerical and logical operations. We believe that our contributions, including defining the problem \hs{is defining the problem our contribution, given the previous work?}, developing our metric, introducing two test sets, and providing insights into the challenges and potential directions for future work, will help lay the foundation for future studies on this important evaluation task.

==> 1_Introduction_v2.tex <==
\section{Introduction}

Generative large language models (LLMs) \cite[inter alia]{brown2020language,ouyang2022training,wei2022finetuned,chowdhery2022palm,openai2023chatgpt,openai2023gpt4,touvron2023llama} often struggle with producing factually accurate statements, resulting in hallucinations \cite{maynez2020faithfulness,ji2023survey}. Such hallucination can be a serious problem, especially in high-stakes domains such as healthcare \cite{nature_medicine_2023,lee2023benefits,lee2023AI} and finance \cite{wu2023bloomberggpt}, where factual accuracy is essential. 

Recent efforts aim to alleviate the hallucination problem by augmenting LLMs with external tools \cite{schick2023toolformer} such as retrievers \cite{shuster2021retrieval,izacard2021leveraging,borgeaud2022improving} and search engines \cite{nakano2021webgpt,thoppilan2022lamda,shuster2022blenderbot}. By incorporating external references to generate the statement, it inherently implies that the statement is backed by the reference. However, the validity of such attribution remains questionable.

% \hs{where [explain how they work..by providing external references for the generation],} 

Inaccurate attribution not only compromises the trustworthiness of LLMs but also raises considerable safety risks and potential harm. For example, in healthcare, an LLM could attribute a generated wrong medical statement to a credible source, potentially misleading users to make harmful health decisions. Similarly, in finance, hallucinated investment advice attributed to a reputable source could result in significant financial losses. In particular, \citet{liu2023evaluating} find that state-of-the-art generative search engines such as XX YY are far from perfect, with only 51.5\% of generated content\nop{ from four generative search engines} fully supported by their cited references. In light of the possible harmful repercussions, accurate attribution is of utmost importance.\footnote{The word ``attribution'' in this paper primarily refers to  ``the act of attributing something''. ``Evaluating attribution'' is the same as ``evaluating verifiability'' in \cite{liu2023evaluating}. }  

%However, evaluating attribution \cite{rashkin2021measuring,gao2022attributed,bohnet2022attributed} is fraught with challenges. 
To evaluate attribution, current methods \cite{rashkin2021measuring,gao2022attributed,bohnet2022attributed} largely depend on human verification, which is both costly and time-consuming. As an illustration, annotating a single (query, answer, reference) example incurs an average cost of about \$1 in \citet{liu2023evaluating}. Moreover, in real use of generative search engines, it is the user who needs to be wary of the attribution and manually verify it, which puts tremendous burden on their side. Therefore, we envision effective, reliable, automatic evaluation methods to measure LLM attribution is highly desired in the future. 

%Hence, the need for effective, reliable, automatic evaluation methods to measure LLM attribution is more urgent than ever.

\begin{figure*}[!t]
    \centering
    \includegraphics[width=\linewidth]{figures/AttrScore.pdf}
    \caption{\score~automatically evaluates attribution by LLMs. We show two recipes for implementing \score: (1) prompting LLMs, and (2) fine-tuning smaller LMs on repurposed datasets from related tasks. }
    \label{fig:attributionscore}
\end{figure*}

% \hs{the box in the middle `attributionscore' should be changed. The icon of `scale' might be changed to that of `lens'.}

% To address these challenges, we present \score, a system designed to automatically evaluate and identify specific types of attribution errors. \score categorizes errors into two types: contradictory errors, where the generated statement directly contradicts the cited reference, and extrapolatory errors, where there is insufficient information in the reference to support the correctness of the generated statement. \hs{we should add 1 or 2 sentences stressing the difference between our catogories and existing ones}

To address these challenges, we present \score (Figure \ref{fig:attributionscore}), a framework designed to automatically evaluate attribution and identify specific types of attribution errors, advancing beyond the binary categorization (i.e., attributable or not) in previous work \cite{rashkin2021measuring,bohnet2022attributed}. Specifically, \score categorizes errors into two types: contradictory errors, where the generated statement directly contradicts the cited reference, and extrapolatory errors, where there is insufficient information in the reference to support the generated statement. Also unlike \citet{liu2023evaluating}, which focuses on the degree of reference support to the generated statement as ``full'', ``partial'', or ``no support'', our classification highlights specific error types in attribution evaluation. \textbf{Such a granular error categorization not only aids users in understanding potential error types that an attributed LLM may generate, improving the safe use of the system, but also offers insightful information for future LLM training, promoting the creation of specialized mechanisms to correct these errors.}



Our implementation of \score explores two approaches: prompting LLMs and fine-tuning smaller LMs on repurposed data from similar tasks such as question answering (QA), fact-checking, natural language inference (NLI), and summarization. For evaluation, \hs{in addition to using a simulated test set,} we curate a set of test examples covering 12 different domains from the generative search engine New Bing \footnote{\url{https://www.bing.com/new}}. \hs{I think we should stress on the importance of this dataset.} \textbf{This is the first evaluation set for LLM attribution with queries newly created based on real-life interactions and hence avoiding the data contamination issue.}

% \hs{minor: should we call it New Bing or Bing Chat (which I think I saw in Stanford or Princeton's paper?)?}.

Our quantitative results indicate that both methods show reasonable performance on our curated and simulated test sets. However, our qualitative analysis reveals that automatic evaluation of attribution is very challenging. Major sources of evaluation failures include insensitivity to fine-grained information comparisons, such as overlooking contextual cues in the reference, disregard for numerical values, and failure in performing symbolic operations such as verifying set relationships.

In light of these findings, we propose potential directions for improving \score, including training \score to be more strongly conditioned on the reference, and augmenting the evaluation with external tools for different types of numerical and logical operations. With the development of \score, the introduction of two test sets, and the insights into challenges and potential directions for future work, we hope our work can help lay the foundation on the important task of automatically evaluating attribution. %to lay the groundwork for future studies on the important task of evaluating attribution in LLMs.









==> 2_Formulation.tex <==
\section{Task Formulation}
Following the work by \citet{rashkin2021measuring} and \citet{bohnet2022attributed}, we define the task of evaluating attribution as  to verify whether the reference  provides sufficient support for the generated output to a user's query. We propose to extend the binary verification \cite{bohnet2022attributed} to a more fine-grained level by classifying input examples into one of three categories:

\begin{itemize}[leftmargin=*]
\item \textbf{Attributable}: The reference fully supports the generation of the query.
\item \textbf{Extrapolatory}: The reference does not provide enough information to determine the correctness of the generation.
\item \textbf{Contradictory}: The generation contradicts the reference.
\end{itemize}

For instance, in the Contradictory example in Figure \ref{fig:attributionscore}, the query \textit{``What was the unemployment rate in Germany in 2020?''} yields an answer of \textit{``4.31\%''}, while the reference indicates that it was actually \textit{``3.81\%''}. In the Extrapolatory example, the reference is relevant to the query but does not provide information on the \textit{``gas price in California''}, thus making it impossible to determine the correctness of the generated answer based on the given information.


Formally, the attribution evaluation task involves a natural language query $q$, an answer $a$, and a reference $x$, where $a$ and $x$ are generated by an attributed LLM. The objective is to develop a score function $f$ that takes $(q,a,x)$ as input and outputs a class label indicating whether ``according to $x$, $a$ of $q$ is correct or not'' \cite{rashkin2021measuring}.\footnote{Note that the attribution evaluation only focuses on the ``verifiability'' of $a$ based on $x$ and does not reflect the ``relevance'' of $a$ to the query $q$, i.e., whether $a$ can actually answer the query $q$ \cite{liu2023evaluating}.} Specifically, $f(q,a,x)=1$ if $a$ is correct (Attributable), $f(q,a,x)=0$ if there is insufficient information in $x$ to verify $a$ (Extrapolatory), and $f(q,a,x)=-1$ if $a$ is incorrect (Contradictory).\hs{(1) I guess this formulation can explain to what the `score' is in `AttributionScore', but since we also mention it is a classification task, what if we formulate as a standard 3-class classification problem, i.e., to predict the probability distribution over three labels using the cross-entropy loss function? (2) in our current formulation, how to determine the label at inference? is it based on which label the score is closest to?}




% \subsection{Traditional NLG Evaluation Metrics}
% In this section, we will discuss how traditional natural language generation (NLG) evaluation metrics are inadequate for this task. Traditional metrics, such as counting the number of overlapping $n$-grams between the generated statement and reference \cite{shuster2021retrieval, peng2023check}, are inadequate for evaluating the attribution. For instance, in the Contradictory example shown in Figure \ref{fig:attributionscore}, many of the tokens in the generation and reference are overlapped, but the critical information \textit{``4.31\%''} in the generation contradicts \textit{``3.81\%''} in the reference. Additionally, one can calculate embedding similarity \cite{zhang2020bertscore, reimers2019sentence, sellam2020bleurt} between the generated text and the reference. However, a high similarity score does not necessarily indicate the accuracy of attribution since it only reflects the semantic relevance between the two texts.

% \subsection{Traditional NLG Evaluation Metrics}
% \paragraph{N-gram Matching} metrics evaluate NLG by counting the number of $n$-grams that occur in both the reference text and the candidate text, such as BLEU \cite{papineni2002bleu}, ROUGE \cite{lin2004rouge}, and METEOR \cite{banerjee2005meteor}. In the context of attribution evaluation, one could count the number of overlapped $n$-grams between the generated output and cited evidence, as in the ``Knowledge F1'' score proposed in \cite{shuster2021retrieval,peng2023check}. However, relying solely on such n-gram matching metrics is not ideal for evaluating the attribution of generations. For instance, in the Contradictory example in Figure \ref{fig:attributionscore}, the ``Knowledge F1'' score would be high, as most of the tokens are overlapped, but the key information \textit{``2021''} in the generation contradicts \textit{``2022''} in the cited evidence. This illustrates that $n$-gram matching metrics are not sufficient to capture the nuances of attribution evaluation.

% \paragraph{Embedding Matching} metrics, such as BERTScore \cite{zhang2020bertscore} and its variants \cite{reimers2019sentence,gao2021simcse,sellam2020bleurt}, use pre-trained LMs to compute a similarity score on contextualized embeddings of a given input text pair. These metrics can be used in the attribution evaluation task to compare the similarity between the generated text and the cited evidence. However, it is important to note that a high similarity score does not necessarily indicate the accuracy of attribution, as it only reflects the semantic relevance between the two texts. More nuanced comparisons are required to determine the accuracy of attribution. For instance, in Figure \ref{fig:attributionscore}, both the Extrapolatory and Contradictory cases may achieve high embedding matching scores despite being negative cases.


\subsection{Connection to Related Tasks}
\label{sec:related_tasks}
In this section, we discuss how this evaluation task is connected to other similar NLP tasks.

\noindent\textbf{Open-domain QA} aims to answer a given question based on a list of retrieved documents \cite{chen2017reading}. However, in traditional open-domain settings, the focus is mostly on the answer's relevance or accuracy rather than evaluating whether the answer is attributed to the retrieved documents. Previous work \cite{bohnet2022attributed} also highlights that a QA model with high accuracy may not necessarily achieve high attribution.

\noindent\textbf{Fact-checking} involves verifying the truthfulness of claims or statements based on retrieved or provided evidence \cite{thorne2018fever}. While our task of attribution evaluation shares similarities with fact-checking in assessing whether the evidence can support or refute a claim, 
%it differs in the type of claim being evaluated. Fact-Checking primarily deals with claims that are factual assertions, personal opinions, beliefs, or interpretations of events. In contrast, the attribution task generates a "claim" from an LLM, which can derive information from both parametric knowledge and external evidence. Both tasks evaluate the credibility of evidence, but 
fact-checking is more concerned with verifying the accuracy of the claim itself, whereas the attribution task focuses on evaluating whether the reference supports the generated text.

\noindent\textbf{NLI} is a task that aims to determine if a given statement (``premise'') logically entails, contradicts, or is neutral with respect to another statement (``hypothesis'') \cite{bowman2015large}. While both NLI and attribution evaluations involve assessing the relationship between two sentences, they differ in focus. NLI primarily concerns the ``logical'' relationship between the premise and hypothesis, with the premise typically being very short. Conversely, attribution evaluation concentrates on verifying whether fine-grained information in the reference supports the generation, with the reference typically being a lengthy document.

\noindent\textbf{Summarization} refers to the task of producing a shorter version of a longer document that preserves the essential information and overall meaning. Hallucinations in summarization systems are classified into two categories \cite{ji2023survey}: 1) \textit{Intrinsic} hallucinations, where the summary contradicts information from the input text; and 2) \textit{Extrinsic} hallucinations, where the model generates information not present in the input text. The detection of hallucinations in summarization is similar to that of attribution evaluation. However, attributed LLMs operate in a query-aware setting where outputs are generated to answer user queries, as opposed to simply producing summaries.

% \vspace{5pt}
% Previous work \cite{gao2022attributed,bohnet2022attributed} builds evaluation models from related tasks such as NLI to generate a score between 0 and 1, indicating the degree of entailment between the reference and the answer to the query. In this work, we extend such methods and study attribution evaluation in a more comprehensive (we extend the binary verification to three-way classification) and realistic manner (we report the performance of evaluation models on curated examples from a generative search engine instead of open-domain QA systems in \cite{bohnet2022attributed}). In the next section, we introduce how we repurpose and simulate examples for training and evaluating \score.

Previous work \cite{gao2022attributed,bohnet2022attributed} develop evaluation models based on NLI datasets to generate scores indicating the degree of entailment between reference and query answers on a scale of 0 to 1. In this work, we extend such methods by employing a three-way classification instead of binary verification and testing evaluation models on curated examples from a real-life generative search engine, rather than open-domain QA systems \hs{people might ask why don't you also evaluate in this setting? We should say sth here.} as done in \cite{bohnet2022attributed}. 

==> 3_AttrScore_v2.tex <==
igure*}[!t]
    \centering
    \includegraphics[width=\linewidth]{figures/Err_Sim.pdf}
    \caption{Examples simulated from open-domain QA. We 1) use the original (question, answer, context) pair as an \textit{attributable} instance \textbf{(A)}, 2) substitute the answer or the answer span in the context to simulate a \textit{contradictory} error example \textbf{(B, C)}, and 3) replace the context with alternatives to simulate an \textit{extrapolatory} error example \textbf{(D)}. In order for \score to generalize well to the long answer setting in real-life search engines like New Bing, we convert the short answer to a long one (using ChatGPT).}
    \label{fig:err-sim}
\end{figure*}

\section{\score}
In this section, we present two approaches for constructing \score to evaluate attribution: prompting LLMs for \score and fine-tuning LMs for \score. 
% \hs{`as' or `for'? like ``Prompt LLMs for \score''?}

\subsection{Prompting LLMs for \score}
Recent research \cite{fu2023gptscore} has demonstrated the possibility of prompting LLMs to evaluate the quality of generated text using their emergent capabilities \cite{wei2022emergent}, such as zero-shot instruction \cite{wei2022finetuned} and in-context learning \cite{brown2020language}. Following this approach, we prompt LLMs, such as ChatGPT \cite{openai2023chatgpt}, using a clear instruction that includes definitions of the two types of errors (as shown in Figure \ref{fig:attributionscore}) and an input triple of the query, answer, and reference for evaluation. The complete prompt used in our study can be found in Appendix Table \ref{tbl:sensitivity_prompt}.

\subsection{Fine-tuning LMs for \score}
\label{sec:finetuned_attrscore}
We also explore fine-tuning LMs of various sizes for this task, ranging from 340M (e.g., Roberta-Large \cite{liu2019roberta}) to 7B (e.g., Alpaca \cite{alpaca}). The primary challenge in fine-tuning \score is the lack of attribution error datasets. One potential approach is to hire annotators to collect error samples, but the cost can be prohibitive (e.g., \$1 per sample, as reported in \citet{liu2023evaluating}). 

Given the connections with those related tasks discussed in Section \ref{sec:related_tasks}, we propose to collect simulated examples by leveraging their benchmark datasets.

% \noindent\textbf{Open-domain QA} benchmarks are one ideal source of data simulation since we have questions, and their ground truth answers and reference contexts, which can be directly used as ``Attributable'' examples (Figure \ref{fig:err-sim}, \textbf{A}). To simulate Contradictory errors, we consider two methods: 1) modifying the correct answer by replacing it with a different candidate generated from an off-the-shelf QA model, an answer substitution model (which outputs a similar phrase to the original answer), or a random span generator (Figure \ref{fig:err-sim}, \textbf{B}), and 2) keeping the original answer and replacing the answer span 
% in the reference context with a similar candidate, which intends to construct instances where the answer would potentially contradict with the internal knowledge \hs{do we have to introduce `internal knowledge' here? I think it is not necessary. (B) could also be conflicting with 'internal knowledge'.} of LMs (Figure \ref{fig:err-sim}, \textbf{C}).
% To simulate Extrapolatory errors, we input the question into a BM25 retriever to retrieve relevant external documents that do not contain ground truth answers from knowledge sources such as Wikipedia or the Web (Figure \ref{fig:err-sim}, \textbf{D}). The answers in the open-domain QA datasets are usually short text spans. \hs{I think this sentence should be brought up earlier and see an earlier comment on `answer span': To accommodate the long answer setting in most attributed LLMs, we convert the short answers to long sentences using ChatGPT.} Additional details on how we simulate these types of errors from QA datasets can be found in Appendix \ref{apdx:error_simulation}. 

\noindent\textbf{Open-domain QA} benchmarks provide an ideal platform for data simulation, as they comprise questions, their corresponding ground truth answers, and reference contexts. These elements can be directly employed as ``Attributable'' examples (Figure \ref{fig:err-sim}, \textbf{A}). In open-domain QA datasets, answers are typically brief text spans. To cater to the long answer setting in most attributed LLMs, we convert these short answers into longer sentences using ChatGPT. For simulating \textit{contradictory} errors, we propose two methods: (1) The first involves modifying the correct answer with an alternative candidate from an off-the-shelf QA model, an answer substitution model, or a random span generator (Figure \ref{fig:err-sim}, \textbf{B}). (2) The second retains the original answer but replaces the answer span in the reference context with a comparable candidate (Figure \ref{fig:err-sim}, \textbf{C}). To emulate \textit{extrapolatory} errors, we employ a BM25 retriever on the question, retrieving relevant external documents from resources like Wikipedia or the Web, which do not contain the ground truth answers (Figure \ref{fig:err-sim}, \textbf{D}). Additional information regarding the simulation of these errors from QA datasets can be found in Appendix \ref{apdx:error_simulation}.

\noindent\textbf{Other related tasks: fact-checking, NLI, and summarization.} Training attribution evaluation models exclusively on our simulated examples using QA datasets may result in over-fitting. Therefore, we investigate the possibility of expanding our simulated examples with data instances from other related tasks, which can be adapted for attribution evaluation by modifying their label space. These tasks include fact-checking, natural language inference, and summarization. Additional information on this can be found in Appendix \ref{apdx:error_simulation}.

% or mode collapsing to the types of attribution errors that we simulate\hs{this last part isn't precise, right? what do we mean exactly? `The types of attribution errors that we simulate' have covered all three types, right? do we mean collapsing to the most frequent types?}

==> 3_AttributionScore.tex <==
\section{\score}
The aim of this study is to develop an evaluation metric ``\score'' for assessing the verifiability of attributed LLMs. In this section, we present two approaches for constructing \score to identify two types of errors and evaluate the attribution: ``Prompt LLMs as \score'' and ``Fine-tune LMs as \score''.

\subsection{Prompt LLMs as \score}
Recent research \cite{fu2023gptscore} has demonstrated the possibility of prompting LLMs to evaluate the quality of generated text using their emerging capabilities \cite{wei2022emergent}, such as zero-shot instruction \cite{wei2022finetuned} and in-context learning \cite{brown2020language}. Following this approach, we prompt LLMs, such as ChatGPT \cite{openai2023chatgpt}, using a clear instruction that includes definitions of the two types of errors (as shown in Figure \ref{fig:attributionscore}) and an input triple of the query, answer, and reference for evaluation. The complete prompt used in our study can be found in Appendix Table \ref{tbl:sensitivity_prompt}.

\subsection{Fine-tune LMs as \score}
\label{sec:finetuned_attrscore}
Although LLMs can act as \score with clear instructions, our preliminary results suggest that their performance is not as expected. To enhance the accuracy of attribution evaluation, we fine-tune LMs of various sizes for this task, ranging from 340M (e.g., Roberta-Large) to 7B (e.g., Alpaca). The primary challenge in fine-tuning \score is the scarcity of attribution error data. One potential approach is to hire annotators to collect error samples \cite{liu2023evaluating}, but the cost can be prohibitive (e.g., \$1 per sample, as reported in \cite{liu2023evaluating}). We propose to generate simulated error examples from the four relevant tasks discussed in Section \ref{sec:related_tasks}.

\noindent\textbf{Data Simulation - QA.} 
We consider (Open-domain) QA, where the answer can be supported by a provided or retrieved document. We construct attributable cases by using the original question, answer, and context in the QA datasets. To simulate Contradictory errors, we consider two methods: 1) modifying the correct answer by replacing it with a different candidate generated from an off-the-shelf QA model, an answer substitution model, or a random span generator, and 2) modifying the answer span in the context by replacing it with a similar candidate. To simulate Extrapolatory errors, we use a retriever to retrieve external documents that do not contain ground truth answers from knowledge sources such as Wikipedia or the Web. Additional details on how we simulate these types of errors from QA datasets can be found in Appendix \ref{apdx:error_simulation}.

\noindent\textbf{Data Simulation - Fact-checking.} Fact-checking involves determining the accuracy of a statement based on provided evidence. In our approach, we concatenate the claim and evidence in the original dataset as text input and map the three labels in fact-checking datasets (``Supported'', ``Refuted'', and ``Not Enough Information'') to ``Attributable'', ``Contradictory'' and ``Extrapolatory'', respectively.

\noindent\textbf{Data Simulation - NLI.} NLI seeks to determine the relationship between two sentences: the ``hypothesis'' and the ``premise''. In our method, we treat the ``hypothesis'' as the claim and the ``premise'' as the evidence. We map the three labels in NLI datasets (``Entailment'', ``Not Entailment'', and ``Neutral'') to ``Attributable'', ``Contradictory'' and ``Extrapolatory'', respectively.

\noindent\textbf{Data Simulation - Summarization.} Summarization systems often face issues of hallucination, both intrinsically and extrinsically. To address this, we consider the summary as the claim and the source text as the evidence. We map the ``golden summary'', ``intrinsic hallucination'', and ``extrinsic hallucination'' in some annotated summarization error datasets to ``Attributable'', ``Contradictory'' and ``Extrapolatory'', respectively, in our approach.

==> 5_Results.tex <==

\begin{table*}[!t]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{p{45mm}Q{15cm}}
\toprule
     \textbf{Error Type (percentage \%)} & \textbf{Example}\\
     \midrule
     Overlooking contextual cues\newline (79.4\%) & 
      \textbf{Query:} Was ketchup a medicine before? 
     
     \textbf{Answer:}: \colorbox{pink}{Yes, that’s true!} Ketchup was sold as a remedy for indigestion, diarrhea, jaundice and rheumatism in the 1830s
     
     \textbf{Reference:} Decades later, in the 1870s, American entrepreneur Henry Heinz created a modern version of ketchup with ripe tomatoes, distilled vinegar, brown sugar, salt and a variety of spices. By 1905, the company had sold five million bottles of ketchup, cementing its place as the condiment we know and love today.

     \textbf{Ground Truth:} Extrapolatory
     
     \textbf{\score:} Attributable. The reference supports the claim that \colorbox{pink}{ketchup was sold as a} \colorbox{pink}{remedy} for various ailments in the 1830s, \colorbox{pink}{indicating that it was used as a medicine before.}  \\
     \midrule
     Fine-grained information \newline  insensitivity\newline (13.8\%) & 
     \textbf{Query:} How many total miles of coastline does Norway have? 
     
     \textbf{Answer:} The official length was recalculated in 2011 as \colorbox{pink}{100,915 km}, including fjords and islands.
     
     \textbf{Reference:} A straight line along Norway's sea borders (the coastal perimeter) is 2,650 kilometers (1,650 mi) long. Along the coast there are many fjords, islands, and bays, resulting in a low-resolution coastline of over \colorbox{pink}{25,000 kilometers} (16,000 mi).

      \textbf{Ground Truth:} Contradictory
      
     \textbf{\score:} Attributable. The reference provides information that the official length of Norway's coastline, including fjords and islands, is \colorbox{pink}{100,915 km}. Therefore, the claim that Norway has a total of 100,915 km of coastline is supported by the Reference. \\
     \midrule
     Failing on symbolic operators\newline (6.8\%) & 
     \textbf{Query:} Is Andrew Ng an author of the recent paper ``generative agents: interactive simulacra of human behavior''? 
     
     \textbf{Answer:} \colorbox{pink}{Yes, Andrew Ng} is one of the authors of the paper ``Generative agents: Interactive simulacra of human behavior''. 
     
     \textbf{Reference:} Computer Science > Human-Computer Interaction [Submitted on 7 Apr 2023] Generative Agents: Interactive Simulacra of Human Behavior \colorbox{pink}{Joon Sung Park, Joseph C. O'Brien,} \colorbox{pink}{Carrie J. Cai, Meredith Ringel Morris, Percy Liang, Michael S. Bernstein}.

     \textbf{Ground Truth:} Contradictory
     
     \textbf{\score:} Attributable. The reference clearly states that Andrew Ng is one of the authors of the paper "Generative Agents: Interactive Simulacra of Human Behavior", which supports the claim that he is an author of the paper. \\
     \bottomrule
\end{tabular}}
\caption{Qualitative analysis on misclassified examples from prompting ChatGPT as \score }
\label{tbl:qual}
\end{table*}


\section{Results}
\label{sec:results}
\subsection{Overall Performance}
\label{sec:result_simulation}

Table \ref{tbl:results_overall} presents an evaluation of different models' performance on both the simulated dataset (AttrEval-Simulation) and annotated dataset on New Bing (AttrEval-GenSearch). Our primary findings are as follows:


\noindent\textbf{Automatic attribution evaluation presents substantial challenges.} This complex task requires not only understanding the reference information but also comparing it with the information in the statement, all of which can significantly vary across different datasets and testing conditions. In the face of these challenges, the overall performance of models in zero-shot, few-shot, and fine-tuning scenarios remained suboptimal. In the simulated test set, language models demonstrated an average F1 score of approximately 60\%, which dipped to around 55\% on the AttrEval-GenSearch test set. Notably, models that yielded impressive results on the simulated test set were less effective on the annotated test set, indicating a lack of consistency across diverse testing conditions - a signal of a generalizability issue.




\noindent\textbf{Fine-tuned smaller models may outperform LLMs.} While LLMs like ChatGPT typically outperform fine-tuned models on many NLP benchmarks \cite{qin2023chatgpt}, our results show that a FLAN-T5-Large model fine-tuned on four repurposed datasets can surpass ChatGPT on both test sets. This implies that fine-tuning smaller LMs could be more effective for difficult unseen tasks.

\noindent\textbf{Larger model size does not ensure superior performance.} Our study contradicts the expectation that larger models always perform better. For example, the smaller FLAN-T5-Large model (770M) outperforms the larger Alpaca model (7B) on the AttrEval-GenSearch set. This suggests that model size is not the only determinant of performance, but pre-training or instruction tuning on similar tasks can also enhance a model's generalizability (see Section \ref{sec:influence_prompt_tuning} for more analysis).

\noindent\textbf{Combining datasets generally enhances performance.} We evaluated the performance of models fine-tuned on individual task datasets and their combinations. Our findings suggest that examples from the fact-checking task most significantly improve performance for the attribution evaluation task, hinting at a strong link between these tasks. Furthermore, integrating various related task datasets generally leads to better performance, particularly on out-of-domain test instances in AttrEval-GenSearch.




% \section{Results}
% \label{sec:results}
% \subsection{Overall Performance}
% \label{sec:result_simulation}
% We first report the overall evaluation performance of different models on both the simulated dataset and annotated dataset on New Bing in Table \ref{tbl:results_overall}. We summarize our key findings as follows:

% \noindent\textbf{The automatic evaluation of attribution poses significant challenges.} We assess the performance of various models in zero-shot, few-shot, and fine-tuning scenarios. Despite the varying strategies, general performance remains suboptimal. On the simulated test set, language models demonstrate an average performance of approximately 60\% F1 score. This performance dips to around 55\% on the AttrEval-GenSearch test set, underscoring the intricacy of the task. Furthermore, an intriguing pattern has emerged - models that excel better in the simulated test set may underperform in the annotated test set. This divergence indicates a generalizability issue, underscoring the challenge of fine-tuned models that can consistently perform well across various testing conditions and datasets.



% \noindent\textbf{Fine-tuning smaller models on repurposed datasets can outperform LLMs.} Previous studies have shown that LLMs like ChatGPT can outperform fine-tuned models on many NLP benchmark tasks \cite{qin2023chatgpt}. However, our results demonstrate that a FLAN-T5-Large model fine-tuned on a combination of four repurposed datasets can outperform ChatGPT on both test sets. This suggests that for such a challenging unseen task, fine-tuning smaller LMs may be a more effective solution than prompting LLMs directly.


% \noindent\textbf{Model size does not always guarantee better performance.}
% Contrary to expectations, our study shows that the largest fine-tuned models, such as Alpaca (7B), do not always achieve the best performance. In contrast, a significantly smaller model, FLAN-T5-Large (770M), achieves the best overall performance on the AttrEval-GenSearch set. This finding suggests that increasing the model size does not necessarily lead to better performance. Other factors such as pre-training or instruction tuning on similar tasks may also contribute to better generalizability of the models (see more analysis in Section \ref{sec:influence_prompt_tuning}).

% \noindent\textbf{Performance generally improves when combining datasets.} Our study probes the performance of fine-tuned models on individual task datasets as well as their combinations. We discern that examples from the fact-checking task are the most beneficial for the attribution evaluation task, suggesting a strong relevance between these two tasks. More importantly, integrating different related task datasets generally boosts performance, especially on out-of-domain test instances in AttrEval-GenSearch.


\subsection{Qualitative Analysis}
\label{sec:qualitative_analysis}
Since ChatGPT predictions are accompanied by explanations, we qualitatively examine some error examples of it to shed light on the space for future improvements in prompting LLMs and potentially also fine-tuning LMs for attribution evaluation. We focus on the zero-shot setting under the attribution prompt. 

Our first observation is that a significant portion (79.4\%) of errors happen due to ChatGPT overlooking the context clues and does not make judgments by conditioning on the reference (e.g., potentially relying on its own parametric knowledge).
For the remaining error cases, they are: 1) fine-grained information insensitivity (13.8\%): failure in comparing over fine-grained information such as numerical values, numbers, dates, and time; 2) failure in performing symbolic operations (6.8\%): the model fails to verify the claim which requires performing symbolic operations over the Reference, such as verifying set relationships. 
Examples for each error category are shown in Table \ref{tbl:qual}. 


Overall, our observations point to two potential directions for improving \score: 1) training or prompting models to be more faithful and strongly conditioned on the reference, as also explored in recent work \citep{zhou2023contextfaithful}; and 2) augmenting an LM-based evaluation method with external tools for different types of numerical and logical operations that are hard to be accurately performed only by the LM itself \citep{Chen2020Neural, mialon2023augmented}.

% \hs{I feel the percentages in Table 3 can be confusing, as they are computed among the remaining 30\% examples, right? and the 70\% errors mentioned above are also largely due to the second type?}

\begin{table}[!t]
\small
\centering
\begin{tabular}{@{}llcccc@{}}
\toprule
\multirow{2}{*}{Models} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Task \\ Prompts\end{tabular}} & \multicolumn{2}{c}{Zero-shot} & \multicolumn{2}{c}{Few-shot} \\ \cmidrule(l){3-6} 
 &  & Sim. & Gen. & Sim. & Gen. \\ \midrule
\multirow{5}{*}{Alpaca} & Attr. & 34.8 & 34.4 & 31.3 & 33.5 \\
 & NLI & 32.1 & 35.5 & 32.1 & 33.6 \\
 & Fact. & 34.0 & 33.9 & 32.7 & 46.7 \\
 & Sum. & 33.6 & 33.5 & 31.6 & 34.8 \\ \cmidrule(l){2-6} 
 & Average & 33.6 & 34.3 & 31.9 & 37.2 \\ \midrule
\multirow{5}{*}{ChatGPT} & Attr. & 37.2 & 45.1 & 37.6 & 51.4 \\
 & NLI & 45.0 & 61.7 & 35.8 & 56.1 \\
 & Fact. & 44.8 & 54.9 & 43.2 & 54.9 \\
 & Sum. & 45.6 & 58.1 & 40.2 & 50.6 \\ \cmidrule(l){2-6} 
 & Average & 43.2 & 55.0 & 39.2 & 53.3 \\ \bottomrule
\end{tabular}%
\caption{Sensitivity of prompts for prompting LLMs as \score on AttrEval-Simulation (Sim.) and AttrEval-GenSearch (Gen.). The prompts include a prompt designed for attribution (Attri.), a prompt based on NLI, a fact-checking prompt (Fact.), and a summarization hallucination detection prompt (Sum.). Fact-checking and NLI prompts generally perform better.}
\label{tbl:sensitivity_prompt}
\end{table}



\subsection{Ablation Study}
\noindent\textbf{Sensitivity of prompts.}
The choice of prompts used to evaluate language models can have an impact on their performance. We evaluate the sensitivity of prompts for \score in both zero-shot and few-shot settings. We show four types of prompts as mentioned earlier: a prompt designed specifically for our evaluation setting (Attri.), an NLI prompt, a fact-checking prompt (Fact.), and a summarization hallucination detection prompt (Sum.). These prompts are presented in Appendix Table \ref{apdx:tbl:sensitivity_prompt}. Based on the results presented in Table \ref{tbl:sensitivity_prompt}, we find that fact-checking and NLI prompts generally perform better, as similar tasks may have been seen during their instruction tuning phase. 

\noindent\textbf{Influence of instruction tuning.}
\label{sec:influence_prompt_tuning}
The purpose of this experiment is to investigate how instruction tuning affects model performance. Results in Table \ref{tbl:instruction_tuning} show that instruction tuning enhances the models' generalizability. Notably, Flan-T5-Large and Alpaca outperform T5-Large and LLaMA, respectively, on AttrEval-GenSearch when instruction tuning is applied. Interestingly, T5-Large outperforms LLaMA, suggesting that the \textit{fill-in-the-blank-style} pre-training objectives may better contribute to the attribution evaluation task
which often requires fine-grained information comparison.



\begin{table}[!t]
\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}lcccc@{}}
\toprule
\multicolumn{5}{c}{AttrEval-Simulation} \\ \midrule
 & Attri. & Contra. & Extra. & All \\\cmidrule(l){2-5}
T5-Large (770M) & 56.4 & 57.5 & 74.7 & 63.2 \\
FlanT5-Large (770M) & 61.5 & 50.4 & 71.9 & 61.5 \\\midrule
LLaMA (7B) & 66.8 & 66.8 & 66.8 & 66.5 \\
Alpaca (7B) & 65.7 & 57.8 & 77.7 & 67.5 \\ \midrule\midrule
\multicolumn{5}{c}{AttrEval-GenSearch} \\ \midrule
 & Attri. & Contra. & Extra. & All\\\cmidrule(l){2-5}
T5-Large (770M) & 55.3 & 29.3 & 73.4 & 62.5 \\
FlanT5-Large (770M) & 63.5 & 34.9 & 74.0 & 65.6 \\\midrule
LLaMA (7B) & 48.9 & 26.3 & 64.8 & 51.8 \\
Alpaca (7B) & 57.4 & 28.6 & 66.4 & 55.0 \\ \bottomrule
\end{tabular}%
}
\caption{Influence of instruction tuning. The results suggest that instruction tuning helps fine-tuned models generalize better in real test scenarios.}
\label{tbl:instruction_tuning}
\end{table}
